Multi-timestep models for Model-based Reinforcement Learning

In model-based reinforcement learning (MBRL), most algorithms rely on simulating trajectories from one-step dynamics models learned on data. A critical challenge of this approach is the compounding of one-step prediction errors as length of the trajectory grows. In this paper we tackle this issue by using a multi-timestep objective to train one-step models. Our objective is a weighted sum of a loss function (e.g., negative log-likelihood) at various future horizons. We explore and test a range of weights profiles. We find that exponentially decaying weights lead to models that significantly improve the long-horizon R2 score. This improvement is particularly noticeable when the models were evaluated on noisy data. Finally, using a soft actor-critic (SAC) agent in pure batch reinforcement learning (RL) and iterated batch RL scenarios, we found that our multi-timestep models outperform or match standard one-step models. This was especially evident in a noisy variant of the considered environment, highlighting the potential of our approach in real-world applications.

==> old_separate_files/Conclusion.tex <==
\section{Conclusion}
\label{sesConclusion}

In this paper, we ask how can we adjust the training objective of $1$-step predictive models to match their ultimate usage, that of generating long rollouts during planning. 
We build on the observation that fixed-horizon models achieve a lower predictive error down-the-horizon, and adapt the idea in the form of a novel training objective for $1$-step models. 
Our idea, \Madd{which materialises in} a weighted sum of the loss function at future prediction horizons, lead to models that when evaluated against noiseless and noisy datasets from the Cartpole benchmark, show a large improvement in r2 compared to the vanilla $1$-step model. 
This improvement translates into better agents in the setting of Offline RL and similar ones in the iterated-batch setup where other confounding factors add-up to the variance of the learning curves. \Gadd{I'd rephrase this, separating the Offline and iterated-batch in two sentences. Maybe for the iterated-batch you can say: that while the method did not give strong advantages in the iterated-batch, it did not lower performance either and future work will analyze what confounding factors did not make performances improve.}

\Madd{I'm wondering whether we should add some text on future work}

\subsection{Limitations}

There are two major limitations of this study that could be addressed in future research. First, the study focused on the Cartpole benchmark, a relatively low-dimensional environment that reduces the modelling complexity that may be encountered in other high-dimensional systems. Nevertheless, to improve the generalisability of our results, we used different offline datasets and considered a more challenging Cartpole variant with additive Gaussian noise. Second, since our proposed objective can be plugged into any single-step model-based algorithm, we believe it would be interesting to test its integration with some of the state-of-the-art MBRL algorithms in different setups/applications. We were not able to do this due to time constraints, but we plan to explore this direction in the near future.



==> old_separate_files/Core.tex <==
\section{Methods}

\subsection{Problem statement}

\Grep{In Model-based Reinforcement Learning (MBRL), we use (very often in the literature)}{In MBRL it is common to use}  models that predict the environment's outcome $1$-step ahead.
We do this by training these models to optimize the $1$-step predictive error (MSE or NLL for stochastic modeling) in a supervised-learning-like setting. 
We then use these models for planning several steps in the future, in order to learn a policy on relatively affordable model-generated traces (as opposed to safety-critical/expensive traces collected on the real system). \Gadd{again I would rephrase without the we. It would make it feel more "objective"}
This is problematic in many ways:
\Gadd{no need to use First of all, Second etc if you're doing a pointed list}
\begin{itemize}
    \item \Grem{First of all,} a distribution mismatch occurs between the inputs that the model was trained on (sampled from the true unknown transition distribution) and the inputs the model being evaluated with (sampled from the model's predicted distribution) \cite{Talvitie_2014, Talvitie_2017}.
    \item \Grem{Second}, the predictive error (and the modeled uncertainty in the case of stochastic models) will propagate through the successive model calls, leading to the \textit{Compounding error effect} \citep{Lambert_2022, Talvitie_2014, Venkatraman_2015}.
    % \item Finally, the model (if not well-calibrated) can be over-confident in regions that are previously unseen in the data, leading to physically unfeasible, and/or safety-violating environment states.
\end{itemize}

% In order to study the relationship between the model's predictive error (both $1$-step ahead and further in the future) and the underlying agent's return, we suggest fixed-horizon models as a starting point.

To mitigate these issues, \Gadd{here the we is nice, as it's us proposing it} we propose to study models that do not simply learn to predict the next state ($s_{t+1}$) given an action $a_{t}$, but those who learn to predict the state ($s_{t+h}$) after an arbitrary future horizon $h$ and the corresponding action sequence $\{a_{t},a_{t+1},\hdots,a_{t+h-1}\}$. One way to achieve this is to align the training objective of the typical 1-step models to their ultimate usage: that of generating long-horizon rollouts.

\Gadd{Add this, or something similar, towards the end of the intro as well to highlight the contributions}
Therefore, we identify two levels in addressing the stated problem:
\begin{enumerate}
    \item Building models that predict the state at a fixed future horizon $h$ (similar to \cite{Whitney_2019})
    \item Adjusting the $1$-step models training objective to account for the error $h$ steps ahead ({\bf our contribution})
\end{enumerate}

We start our analysis from point $1$ in section \ref{secFixedHor}, and address point $2$ in section \ref{secImprove1}. Finally, the experimental setup and the performance evaluation of the agents underlying our proposed models is showcased in section \ref{secExp}.

\subsection{Fixed-horizon models}
\label{secFixedHor}

Fixed-horizon models are neural networks \Gadd{That's not always the case, don't they use Gaussian processes in PETS? You can say something like: the most common type of fixed-horizon models are NN..} that take as input a current state $s_t$, an action sequence $(a_t,a_{t+1},\hdots,a_{t+k-1})$, and predict\Mrem{s} the parameters of a diagonal multi-variate Gaussian distribution over the state observed $k$ steps into the future: $\hat{s}_{t+k} \sim \mathcal{N}(\hat{\mu}_\theta(s_{t+k}|s_t,a_t,a_{t+1},\hdots,a_{t+k-1}), \hat{\sigma}_\theta(s_{t+k}|s_t,a_t,a_{t+1},\hdots,a_{t+k-1}))$ with $\theta$ representing the parameters of the neural network. % To refer to these models, we use the notation $dn\_fixed\_n'k'$ where $dn$ stands for \textit{deep network}. For e.g: $dn\_fixed\_n10$ is a model that predicts the state $10$ steps ahead.

\begin{figure}[htp]
\centering
\includegraphics[width=.475\textwidth]{clean_figures/fixed_cartpole_random.png}
\includegraphics[width=.475\textwidth]{clean_figures/fixed_cartpole_hotp.png}
\includegraphics[width=.8\textwidth]{clean_figures/fixed_legend.png}
\caption{Caption}
\label{fig:fixed}
\end{figure}

Figure \ref{fig:fixed} shows the error at different horizons for different fixed-horizon models and datasets. For each horizon $h$, the error is computed by considering all sub-trajectories of size $h$ from the Test dataset. For a $k$-steps ahead model where $k$ divides $h$, we call the model recursively $h // k$ times to compute the prediction $h$ steps ahead. If $k$ does not divide $h$, we don't consider this particular horizon for this particular model. 

\Gadd{You should say somewhere something about the two datasets (why their names and how they're generated). Even a single sentence is enough}
In general\Gadd{, for a given horizon,} we observe that the r2 \Madd{use a mathematical symbol for r2} score increases as we go from the $1$-step model to the $100$-steps model. For the Cartpole \textbf{random} \Grep{trace}{dataset}, the shorter-horizons models are almost identical, while the $50$-steps and the $100$-steps achieve distinguishable r2 scores. In the \textbf{hot\_purple} \Grep{trace}{dataset} the improvement is rather smooth as every $h$-steps model achieves a larger r2 than its precedents \Madd{I would rephrase the last sentence}.

These results show that the fixed-horizon models can be \Grep{a strong candidate}{strong candidates} to challenge the wide usage of $1$-step models. However, there are some considerations that hinders their practical implementation:
\begin{itemize}
    \item \Grem{First of all,} when using $h$-steps models we do not have access to the intermediate states visited between the input state $s_t$ and the predicted state $h$ steps ahead: $s_{t+h}$. This is problematic because planning algorithms require access to these states in order to evaluate policies/action\_sequences. A potential solution is to predict the return (sum of rewards) cumulated during the prediction scope: $\hat{R_h}(\{a_1,a_2,\hdots,a_h\}) \approx \sum_{i=1}^h r(s_{t+i})$ \Gadd{predict, so through the model? maybe mention the fact that it would be the output of the model}. Another solution is to consider the return of the accessible chunk of the trajectory as a surrogate to the full return: 
    $$
    \Tilde{R}(\{a_1,a_2,\hdots,a_h\}) = \sum_{i=0}^{h//k} r(s_{t+ i \times k}) \approx \sum_{i=0}^{h} r(s_{t+i}) = R(\{a_1,a_2,\hdots,a_h\})
    $$
    \item \Grem{Furthermore,} in the case of noisy environments, the noise accumulates through future timesteps leading to high levels of noise on the learning targets of $h$-steps models. In the case of high values of $h$, we would need a large amount of training data which limits the usability of the fixed-horizon models.
\end{itemize}

Based on the improvement observed in the predictive error of fixed-horizon models, and the considerations that limit their practical usage, we propose a novel training objective to improve the widely used $1$-step models.

\subsection{Improving the $1$-step models with the error $h$-steps ahead}
\label{secImprove1}

\Gadd{maybe add a short sentence to intro the section? It feels weird not to have one imho}

\subsubsection{An example: Optimizing the error $2$-steps ahead}

We start our contribution from the observation that the $1$-step model gets a larger predictive error down-the-horizon than the $2$-steps model Figure \ref{fig:r2_1_2}. 

\begin{wrapfigure}{r}{0.6\textwidth}
\vspace{-5mm}
  \begin{center}
    \includegraphics[width=0.6\textwidth]{clean_figures/fixed_cartpole_l2.png}
  \end{center}
  \vspace{-4mm}
  \caption{Caption}
  \vspace{-5mm}
  \label{fig:r2_1_2}
\end{wrapfigure}

An idea that we can derive from this result is that optimizing the model's predictive error for further horizons \Mrep{help you achieve}{helps achieving} smaller error when planning for very long horizons. 
\Gadd{I would rephrase this to remove the 'An idea..' as it's a bit informal. Maybe something like: 'From this result we can infer that optimizing...'}
In the case of the fixed-horizons models, this is probably due to less compounding errors as the $h=2$ model \Madd{is evaluated} $H//2$ times, while the $1$-step model \Madd{is evaluated} $H$ times for a prediction horizon $H$. 
However, in practice we can attempt a similar improvement by explicitly adjusting the training objective to optimize the error $2$-steps ahead.

Formally, we consider a $2$-steps trajectory: $\mathcal{T} = \{s_t,a_t,s_{t+1},a_{t+1}, s_{t+2},a_{t+2}\}$, a deterministic $1$-step model: $\hat{s}_{t+1} = \hat{f}_\theta(s_t, a_t)$ with parameters $\theta$, and the MSE loss: $\mathcal{L}^1 = (\hat{f}_\theta(s_t,a_t) - s_{t+1})^2$. 

\begin{figure}[htp]
\centering
\includegraphics[width=.475\textwidth]{clean_figures/l2_cartpole_random.png}
\includegraphics[width=.475\textwidth]{clean_figures/l2_cartpole_hotp.png}
\includegraphics[width=.8\textwidth]{clean_figures/l2_legend.png}
\caption{Caption}
\label{fig:soft_r2}
\end{figure}

We define the $2$-steps MSE loss by using a recursive call to the model in order to predict the state after 2 steps \Madd{I think it might be better to denote this as $\mathcal{L}^{(2)}$ instead, to avoid confusion with the square operation - the same notation should be employed for 1-step, h-step etc...}: $$\mathcal{L}^2 = (\hat{f}_\theta(\hat{s}_{t+1},a_{t+1}) - s_{t+2})^2 = (\hat{f}_\theta(\hat{f}_\theta(s_t, a_t),a_{t+1}) - s_{t+2})^2$$
Ideally, we would like the model to achieve small errors both $1$-step, and $2$-steps ahead. Therefore, the immediate learning objective we can think of is the sum of both learning objectives: $\mathcal{L} = \mathcal{L}^1 + \mathcal{L}^2$. 
\Gadd{Rather than saying 'For practical reasons', I would just say that you do a weighted sum of the two losses, otherwise you'll have to mention what those practical reasons are and it would take more space :) }However for practical reasons, we introduce a soft-sum parameter $\alpha$ to control the trade-off between the $1$-step, and the $2$-steps error: $$\mathcal{L} = \alpha \mathcal{L}^1 + (1 - \alpha)\mathcal{L}^2$$

The experiments in Figure \ref{fig:soft_r2} show promising results: \Grep{In}{in} both the \textbf{hot\_purple} and the \textbf{random} datasets, the models where $\alpha < 1.0$ not only recover the predictive error loss \Gadd{what do you mean by 'recover the predictive error loss'? The plots just show the r2 score} between the $1$-step and the $2$-steps models, but they achieve much higher r2-score. 

% It is also worth to mention that unlike \textbf{hot\_purple}, the scale of the differences in r2 is very small in the \textbf{random} dataset. This is usually due to the small variance in the traces collected by a random policy (even after $200$ steps, the cartpole is still exploring the same state space regions as in the beginning).

\subsubsection{Generalization to $\mathcal{L}^h$}

Following the promising empirical results in the previous simple case, we hypothesize that \Grem{the way} to reduce the error of the $1$-step model at an arbitrary planning horizon $h$, \Grep{is by training}{we can train } the model to optimize the error $h$ steps ahead: $\mathcal{L}^h$. 
We can thus imagine a generalization of the soft-summed loss that covers all the intermediate losses up to a maximum horizon $n$ (for simplicity, we omit actions from the inputs of the transition function): 

\begin{equation} \label{eq1}
\mathcal{L} = \sum_{h=1}^n \alpha_h \mathcal{L}^h = \sum_{h=1}^n \alpha_h (\hat{f}_\theta^h (s_t) - s_{t+h})^2 \hspace{.4cm} \text{where } \hat{f}_\theta^h = \hat{f}_\theta \circ \hat{f}_\theta \circ \hdots \circ \hat{f}_\theta \text{ $h$ times,  and }\sum_{h=1}^n \alpha_h = 1
\end{equation}

In practice, we only need the gradient of the loss with respect to the model's parameters to proceed with \textit{gradient descent}-based optimization: $\frac{d}{d \theta} \mathcal{L} = \sum_{h=1}^n \alpha_h \frac{d}{d \theta} \mathcal{L}^h$. We denote the error ratio between horizons $i$ and $j$: $Err_{(i,j)} = \frac{(\hat{f}_\theta^j (s_t) - s_{t+j})}{(\hat{f}_\theta^{i} (s_t) - s_{t+i})}$; And the gradient of the prediction function evaluated at the $i$-th horizon: $G_{i} = \frac{d}{d \theta} [\hat{f}_\theta]\big(\hat{f}_\theta^{i}(s_t)\big)$. Under the assumption of a single-dimensional state and the MSE loss, the formula for the gradient of the generalized loss $\mathcal{L}$ with respect to a parameter $\theta$ is the following (refer to appendix \ref{AppSecGrad} for a detailed derivation):

\begin{equation} \label{eq0}
\frac{d}{d \theta} \mathcal{L}  = \sum_{h=1}^n \alpha_h \frac{d}{d \theta} \mathcal{L}^h = \sum_{h=1}^{n} \alpha_h \left( \prod_{i=0}^{h-1} G_i \right) \left( Err_{(1,h)} \right) \frac{d}{d \theta} \mathcal{L}^1
\end{equation}

We derive the gradient in equation \ref{eq0} to highlight the fact that our proposed method consists in back-propagating the gradient of the loss through the successive compositions of the model ($\hat{f}_\theta^h (s_t)$) that figure in $\gL^h$. Compared to other ideas from the literature (hallucinated replay \cite{Talvitie_2014}, multi-step loss \cite{Byravan_2021}), this is the main novelty of our approach. 
Furthermore, this formulation expresses the generalized loss derivative as a linear function of the derivative of the loss $1$-step ahead. 
The latter is relatively cheap and can be computed with one forward (and backward) pass through the model. 
Consequently, we can think of approximation schemes to reduce the computational burden $O(n \times Cost(\mathcal{L}^1))$ that comes with computing the full derivative: $\frac{d}{d \theta} \mathcal{L}$. 
We leave the \Grep{exploitation}{exploration} of this idea to a future follow-up work.

\subsubsection{How to choose $\{\alpha_h\}_{h \in \{1,\hdots,n\}}$ ?}

The choice of $\alpha_h$ is very important in this context, \Madd{as} it allows us to balance the optimization problem between losses at different prediction horizons. In fact, the different loss terms are at different scales since the error grows with the prediction horizon. \Madd{Maybe add something like: "and therefore a sensible choice of these weights is critical."}

\begin{figure}[ht]
\begin{center}
   \includegraphics[width=.55\linewidth]{clean_figures/weight_profiles.png}
\end{center}
\caption{Caption}
\label{fig:w}
\end{figure}

\begin{itemize}
    \item \textbf{uniform.} $\alpha_h = 1/n$ The most intuitive way to handle the weighting of the losses is by using uniform weights. However, this method can be sub-optimal as the loss terms $\mathcal{L}^h$ have different scales.
    \item \textbf{decay.} $\alpha_h = (\frac{1-\beta}{1-\beta^{n+1}}) \beta^h$ This method implements an exponential decay through a parameter $\beta$ (Figure \ref{fig:w} shows the weight profiles obtained using different values of $\beta$).
    \item \textbf{learn.} $ \alpha_h = learnable $ In this setting, the $\alpha_h$ are left as free-parameters to be learned by the model. The expected outcome in this case is that the model puts the biggest weight on $\mathcal{L}^1$ as it's smaller than further horizons. 
    \item \textbf{proportional.} $\alpha_h = \frac{\frac{1}{\mathcal{L}^h}}{\sum_{h'}^n \frac{1}{\mathcal{L}^{h'}}}$ This method normalizes all the loss terms with their amplitude so that they become equivalent optimization-wise. 
\end{itemize}






==> old_separate_files/Experiments.tex <==
\section{Experiments \& Results}
\label{secExp}
\Gadd{Maybe Add a short sentence here}
\subsection{Experimental setup}

The problem at hand \Madd{Maybe replace with: "The problems we are interested in this work"} can be divided into two separate parts: Model Learning, and Agent learning from model-generated traces. \Gadd{the 'learning' has to be for both either capitalized or not}
While we are interested in building models that improve the predictive error beyond the $1$-step transition, the relationship between this surrogate metric and the return of the underlying agent is not trivial. Indeed, in many scenarios, models that have lower predictive ability lead to better performing agents \citep{Talvitie_2014}. 

Therefore, we suggest the following experimental settings:

\begin{itemize}
    \item \textbf{Offline RL.} In this setting, we dispose of multiple datasets with different characteristics. We then test the predictive error of our models against these datasets in a supervised-learning fashion. The main metric in this setting is the r2 score that we evaluate at different future horizons. The resulting models can then be used to train a RL agent (We use Soft-Actor Critic, implementation details can be found in appendix \ref{appendixsecImpDetails}) in what can be seen as a single-iteration MBRL.
    \item \textbf{Iterated-batch RL.} In this setting, we alternate between generating a system trace (one episode from the real system), training the model using the traces collected so-far, and training the policy (RL agent) on the freshly updated model. 
\end{itemize}

We conduct our experiments in the continuous control environment \textit{Cartpole swing-up}. We use the implementation of Deepmind Control \citep{Tassa_2018} which is based on the Mujoco physics simulator \citep{Todorov2012}. A description of this environment can be found in appendix \ref{appendixcartpole}. A detailed comparison of the static datasets used in the \textbf{Offline RL} setting is given in Appendix \ref{appendixdatasets}.

\paragraph{Noisy Environment} In an effort to further examine the applicability of multi-timestep models, we suggest the use of a \textit{Cartpole swing-up} variant that is characterized by the addition of Gaussian noise with a fixed \Mrep{sigma}{variance} ($\epsilon \sim \gN(0,0.01)$) to all observable variables. The Noisy Cartpole environment is of particular interest due to the potential for multi-timestep models to experience significant failures as a result of the accumulation of substantial noise on the learning targets projected h-steps ahead. We aim to demonstrate that our proposed method effectively addresses this problem by introducing self-consistency through the concurrent optimization of errors for future horizons.

% To further test the usability of multi-timestep models, we propose to use a \textit{Noisy} Cartpole dataset where a Gaussian noise with fixed sigma ($\epsilon \sim \gN(0,\sigma=0.01)$) is added to all the observables. The \textit{Noisy Cartpole} environment is particularly interesting because multi-timestep models may fail drastically because of the high level of noise that accumulates on the $h$-steps ahead learning targets. Therefore, we want to show that our suggested method effectively mitigates this issue through the self-consistency introduced by jointly optimizing for future horizons errors.

\subsection{Static evaluation: r2 on fixed datasets}

For each horizon $h$, the error is computed by considering all the sub-trajectories of size $h$ from the Test dataset. The predictions are then computed by $h$ model compositions (using the groundtruth actions) and the average r2 score is reported.

\begin{figure}[htp]
\centering
\includegraphics[width=.325\textwidth]{clean_figures/lh_2_cartpole_hotp.png}
\includegraphics[width=.325\textwidth]{clean_figures/lh_4_cartpole_hotp.png}
\includegraphics[width=.325\textwidth]{clean_figures/lh_10_cartpole_hotp.png}
\includegraphics[width=.325\textwidth]{clean_figures/lh_2_cartpole_noisy.png}
\includegraphics[width=.325\textwidth]{clean_figures/lh_4_cartpole_noisy.png}
\includegraphics[width=.325\textwidth]{clean_figures/lh_10_cartpole_noisy.png}
\includegraphics[width=.8\textwidth]{clean_figures/lh_legend.png}
\caption{Caption}
\label{fig:alpha}
\end{figure}

Figure \ref{fig:alpha} shows the r2 score as a function of the prediction horizon $h$, when using multiple weight profiles for three maximum horizons \Gadd{models}: $n \in \{2,4,10\}$ \Grem{model}. In both the \textbf{hot\_purple} and \textbf{quicksand\_noisy} \Grep{traces}{datasets}, the multi-timestep models largely improve over the vanilla $1$-step model. 
Depending on the future horizons scope, we obtain different optimal weight profiles (mostly from the noisy dataset as in the noiseless one the differences are minor): $decay(\beta=0.9)$ for $n=2$, $decay(\beta=0.75)$ for $n=4$, and $decay(\beta=0.3)$ for $n=10$. 
We interpret the effectiveness of the $decay$ weighting schema from the error profile witnessed for the $1$-step model. 
Indeed, the error for this model grows exponentially with the prediction horizon (\Grep{A}{a} theoretical justification can be found in Theorem 1 of \cite{Venkatraman_2015}), suggesting that exponentially decaying weights (modulo the right parameter $\beta$) can correctly balance the training objective.

Inspired by this finding, we investigated the direct use of weights that are the exact inverse of the loss term they correspond to ($\alpha_h=proportional$). 
However, this technique didn't further improve the results. 
A potential explanation is the interdependence between the different losses as reducing one loss can indirectly affect another one.

Unsurprisingly, the learnable weighting profile quickly converges to putting most of the weight on the $1$-step error, this is expected because the $1$-step loss is the smallest among the other terms. 
A potential fix to this phenomena is to add a regularization term that enforces the weights to be more equally distributed. 
The elaboration of this idea is beyond the scope of this work.

\subsection{Dynamic evaluation: Offline RL}

To demonstrate the effectiveness of multi-timestep models in practical RL scenarios, we start with the Offline RL setting. Using the \textbf{hot\_purple} dataset for the \textit{Cartpole swing-up} environment, and the \textbf{quicksand\_noisy} dataset for its noisy version, we train SAC agents on models that are themselves trained on these respective datasets. We choose the best model on each maximum horizon ($decay(\beta=0.9)$ for $n=2$, $decay(\beta=0.75)$ for $n=4$, and $decay(\beta=0.3)$ for $n=10$), and the vanilla $1$-step model for comparison.

\begin{table}[!ht]
  \scriptsize
  \vspace{-4mm}
  \caption{Caption. \abdelhakim{yet to update all the numbers}}
  \label{tabDynamic}
  \centering
  \begin{tabular}{lllll}
    \toprule
    Model
    & hot\_purple
    & quicksand\_noisy
    & random \abdelhakim{?}
    & quicksand \abdelhakim{?}
    \\
    \cmidrule(r){1-5}
    $h=1$
    & 31.34 $\pm$ \abdelhakim{0.41}   
    & 17.54 $\pm$ \abdelhakim{7.96}
    & 31.97 $\pm$ \abdelhakim{0.21}
    & 31.97 $\pm$ \abdelhakim{0.21}
    \\
    $n=2|\alpha=decay(\beta=0.9)$
    & 66.96 $\pm$ \abdelhakim{5.14}   
    & 33.12 $\pm$ \abdelhakim{4.84}
    & 14.12 $\pm$ \abdelhakim{10.76}
    & 31.97 $\pm$ \abdelhakim{0.21}
    \\
    $n=4|\alpha=decay(\beta=0.75)$
    & 70.57 $\pm$ \abdelhakim{19.86}   
    & 33.16 $\pm$ \abdelhakim{1.54}
    & 28.96 $\pm$ \abdelhakim{12.89}
    & 31.97 $\pm$ \abdelhakim{0.21}
    \\
    $n=10|\alpha=decay(\beta=0.3)$
    & 64.18 $\pm$ \abdelhakim{20.39}   
    & - $\pm$ -
    & \abdelhakim{32.10} $\pm$ \abdelhakim{0.54}
    & 31.97 $\pm$ \abdelhakim{0.21}
    \\
    \bottomrule
  \end{tabular}
\vspace{-4mm}
\end{table}

\begin{figure}[htp]
\centering
\includegraphics[width=.95\textwidth]{clean_figures/offline_cartpole_hotp.png}
\includegraphics[width=.95\textwidth]{clean_figures/offline_cartpole_noisy.png}
\includegraphics[width=.8\textwidth]{clean_figures/offline_legend.png}
\caption{Caption: \abdelhakim{See if we only keep the table here and move the discussion on the correlation with r2 to some appendix}}
\label{fig:offline}
\end{figure}

Although with high variance due to SAC being trained for only $500k$ steps [\abdelhakim{If we debug the offline issue, update the plots with the correct values}], we observe that multi-timestep models (precisely, the $n=2$ and $n=4$ models) achieve a higher real-environment return than the vanilla $1$-step model. 
The x-axis shows the r2 achieved by the corresponding models\Grep{, it }{. This} gives us a hint on whether the predictive error of the models is correlated with their returns. \abdelhakim{elaborate on this if we keep this plot, if we move to a table then remove this comment} 

% To gain more insights on this, we compute Spearman rank correlation ($\rho$) and Pearson bivariate correlation ($r$) between the r2 score obtained for all models and their respective returns. \abdelhakim{see if we add correlation plot and comment, otherwise remove this last part}

\subsection{Dynamic evaluation: Iterated-batch RL}

\begin{figure}[htp]
\centering
\includegraphics[width=.475\textwidth]{clean_figures/iterated_cartpole.png}
\includegraphics[width=.475\textwidth]{clean_figures/iterated_cartpole_noisy.png}
\includegraphics[width=.8\textwidth]{clean_figures/iterated_legend.png}
\caption{Caption}
\label{fig:iterated}
\end{figure}

Finally, we run the full MBRL loop \Gadd{did you mention somewhere what the full MBRL loop is?} with the best multi-timestep models and compare the results with the vanilla $1$-step models. 
In this setting, the improvement brought by the  multi-timestep models is not significant as the episodic return show a large variance among all the models. 
\abdelhakim{Hypothesize on why is there a large variance and what's the takeaway, waiting for the last seeds to finish}.

==> old_separate_files/Intro.tex <==
\section{Introduction}
\label{secIntroduction}

Reinforcement learning is a paradigm where a control agent, or policy, learns through interaction with a dynamic system, or environment, and receives feedback in the form of rewards. This approach has proven successful in addressing some of the most challenging problems globally, as evidenced by \citep{Silver2017, Silver2018, Mnih2015, Vinyals2019}. However, the application of reinforcement learning remains largely confined to simulated environments and does not extend to real-world engineering systems. This limitation is primarily due to two factors: i) the scarcity of data resulting from operational constraints, and ii) the safety standards associated with these systems. To narrow the gap between reinforcement learning and its application in engineering systems, we motivate the setting of Model-based Reinforcement Learning (MBRL).

Model-based reinforcement learning (MBRL) algorithms consist of two distinct and often alternating phases: i) model learning, which is a supervised learning problem that involves learning the dynamics of the system under consideration, and ii) policy optimization, where a policy and/or a value function is learned by sampling from the learned dynamics. MBRL is recognized for its sample efficiency, as the learning of policy/value is conducted (either wholly or partially) from imaginary model rollouts (also referred to as background planning), which are more cost-effective and readily available than rollouts in the true dynamics \citep{Janner2019}. Moreover, a predictive model that performs well out-of-distribution facilitates easy transfer of the true model to new tasks or areas not included in the model training dataset \citep{Yu2020}.

While model-based reinforcement learning (MBRL) algorithms have achieved significant success, they are prone to \textit{Compounding errors} when planning over extended horizons \citep{Lambert_2022}. This issue arises due to the propagation of model bias, leading to highly inaccurate predictions further down the horizon. This can be problematic in real-world applications, as it can result in out-of-distribution states that may violate the physical or safety constraints of the environment. The root of the \textit{Compounding errors} problem lies in the nature of the models used in MBRL. Typically, these are 1-step predictive models that predict the next state based on the current state and executed action. However, these same models are used to generate long rollouts during planning. To address this issue, we propose aligning the training objective of these models to optimize future horizon-error, resulting in \textbf{Multi-timestep models}.

Our key contributions are the following:

\begin{itemize}
    \item We propose a novel training objective for $1$-step predictive models. It consists in a weighted sum of the loss function at multiple future horizons.
    \item We perform an ablation on different weight profiles finding that exponentially decaying weights lead to the best results.
    \item Finally, we evaluate the multi-timestep models against the offline RL and iterated-batch RL settings.
\end{itemize}

==> old_separate_files/Prelims.tex <==
\section{Preliminaries}

The conventional framework utilized in \textbf{Reinforcement Learning (RL)} is the finite-horizon Markov Decision Process (MDP), denoted as $\mathcal{M} = \langle  \mathcal{S}, \mathcal{A}, p, r, \mu_0, \gamma \rangle$. 
In this notation, $\mathcal{S}$ symbolizes the state space and $\mathcal{A}$ \Grem{signifies} the action space. 
The transition dynamics, which could be stochastic, are represented by $p : \mathcal{S} \times \mathcal{A} \leadsto \mathcal{S}$. The reward function is denoted by $r : \mathcal{S} \times \mathcal{A} \rightarrow \mathbb{R}$. The initial state distribution is given by $\mu_0$ \Gadd{maybe another symbol might be better, as $\mu$ usually means the mean?}, and the discount factor is represented by $\gamma$, and lies within the range of [0,1].

The objective of Reinforcement Learning (RL) is to identify a distribution, known as the policy ($\pi(s)$), over the action space ($\mathcal{A}$) for each state ($s \in \mathcal{S}$). This policy aims to maximize the expected sum of discounted rewards, denoted as $J(\pi, \mathcal{M}) := \mathbb{E}_{s_0 \sim \mu_0, a_t \sim \pi, \, s_{t>0} \sim p}[ \sum_{t=0}^{H} \gamma^t r(s_t, a_t) ]$, where $H$ represents the horizon of the \Grep{Markov Decision Process (MDP)}{MDP}.
Under a given policy $\pi$, the state-action value function (also known as the Q-function) at a specific $(s,a) \in \mathcal{S} \times \mathcal{A}$ pair is defined as the expected sum of discounted rewards. This expectation starts from state $s$, takes action $a$, and follows the policy $\pi$ until termination: $ Q^\pi(s, a) = \mathbb{E}_{a_{t>0} \sim \pi,  s_{t>0} \sim p} \big[ \sum_{t=0}^H \gamma^{t} r(s_t,a_t) \mid s_0=s, a_0=a \big]$. Similarly, we can define the state value function by taking the expectation with respect to the initial action $a_0$: $ V^\pi(s) = \mathbb{E}_{a_t \sim \pi,  s_{t>0} \sim p} \big[ \sum_{t=0}^H \gamma^{t} r(s_t,a_t) \mid s_0=s\big]$.

\textbf{Model-based RL (MBRL)} algorithms utilize a dataset, denoted as $\mathcal{D}$, to address the supervised learning challenge of estimating the dynamics of the environment ($\hat{p}$) and/or the reward function ($\hat{r}$). \Gadd{I would reformulate this, as it seems weird to define MBRL algos as using a dataset. Of course they use it, but I would not use this as their primary definition (you can see the replay buffer of Q learning as a dataset as well)}
The loss function is typically the log-likelihood $\mathcal{L}(\mathcal{D}; \hat{p}) = \frac{1}{N} \sum_{i=1}^N \log  \hat{p}(s^i_{t+1}|s^i_t, a^i_t)$ or Mean Squared Error (MSE) when $\sigma$ is fixed. 
The learned model can subsequently be employed for policy search under the \Grep{Markov Decision Process (MDP)}{MDP} $\hat{\mathcal{M}} = \langle  \mathcal{S}, \mathcal{A}, \hat{p}, \hat{r}, \mu_0, \gamma \rangle$. 
This MDP shares the same state and action spaces $\mathcal{S}, \mathcal{A}$ as the true environment $\mathcal{M}$, but utilizes the transition probability $\hat{p}$ and the reward function $\hat{r}$ learned from the \Grep{data buffer}{dataset} $\mathcal{D}$. The optimal policy obtained, denoted as $\hat{\pi} = \argmax_\pi J(\pi, \hat{\mathcal{M}})$, is not guaranteed to be optimal under the true MDP $\mathcal{M}$ due to factors such as distribution shift and model bias. 

In the context of \textbf{Offline RL},  we are provided with a set of transitions, denoted as $\mathcal{D}=\{(s_t^i,a_t^i,r_t^i,s_{t+1}^i)\}_{i=1}^N$, where $N$ represents the size of the set. These transitions are generated by an unknown behavioral policy, $\pi^\beta$. 
The challenge in offline RL arises from the constraint that \Mrep{we are}{it is} not permitted to further interact with the environment $\mathcal{M}$, despite the fact that \Grep{our}{the} objective is to optimize $J(\pi, \mathcal{M})$ with $\pi \not= \pi^\beta$.

In terms of the model type, the common \Grep{selection}{choice} is a probabilistic model that learns the parameters of a multivariate Gaussian over the subsequent state and reward, conditioned on the current state and action: $ s_{t+1}, r_t \sim \hat{p}_\theta(.| s_t,a_t) = \mathcal{N}\big(\mu_\theta( s_t,a_t),\sigma_\theta( s_t,a_t)\big)$, where $\theta$ denotes the parameters of the predictive model.  \Gadd{is it that common? maybe a reference here can be useful}
In practical applications, fully connected neural networks are often employed due to their proven capabilities as powerful function approximators \citep{Nagabandi2018,Chua2018}, and their suitability for high-dimensional environments over simpler \Mrep{non-parametric}{nonparametric} models such as Gaussian processes. Following previous research \citep{Chua2018}, we assume a diagonal covariance matrix for which we learn the logarithm of the diagonal entries: $\sigma_\theta = \mathrm{Diag}(\exp(l_\theta))$ \Mrep{with $l_\theta$ output by}{where $l_\theta$ denotes the output of} the neural network.

==> old_separate_files/Related_Work.tex <==
\section{Related Work}

\paragraph{Model-based Reinforcement Learning} MBRL has been effectively used in the online RL setting by alternating between model learning and planning \citep{Deisenroth2011,Hafner2021,Gal2016,Levine2013,Chua2018,Janner2019,Kegl2021}, and in the offline RL setting which can be regarded as single-iteration RL \citep{Yu2020,Kidambi2020,Lee2021,Argenson2021,Zhan2021,Yu2021,Liu2021,Benechehab_2023}. 
Planning is executed either decision-time via Model-Predictive Control \Gadd{(MPC)} \citep{Draeger1995,Chua2018,Hafner2019,Pinneri2020,Kegl2021}, or Dyna-style by training a model-free agent on imagined model rollouts \citep{Janner2019,Sutton1991,Sutton1992,Ha2018}. \Gadd{Dyna-style is not really planning, no?}
For example, Model-Based Policy Optimization (MBPO) \citep{Janner2019} trains an ensemble of feed-forward models and generates imaginary rollouts to train a soft actor-critic agent.

\paragraph{Multi-step predictions} Multi-timestep dynamics modeling are partially addressed in MBRL by means of Recurrent state space models \citep{Hochreiter_1997, Chung_2014, Ha2018, Hafner2019, Hafner2021, Silver_2017}. However, these methods rely on heavy computation and approximated inference schemes such as variational inference. The problem of multi-step forecasting was also addressed in the time series literature \citep{Bentaieb_2012a, Bentaieb_2012b, Venkatraman_2015, Chandra_2021}, but none directly aligns the single-step forecasting model training objective to match the multi-step prediction objective as we propose.

\paragraph{Fixed/Variable-horizon architectures} Regarding fixed-horizon models, \cite{Asadi_2018, Asadi_2019} designed a model that has a distinct neural block for each prediction step, which reduces error accumulation but enlarges model size. \cite{Whitney_2019} demonstrated that a simple fixed-horizon model has better accuracy and can be used for planning with CEM. 
However, the latter had to change the reward function to overcome the fact that we \Gadd{I would not use the 'we' form of the verb, it makes it too informal imo} don't have access to all the visited states when planning with a fixed-horizon model (discussed in section \ref{secFixedHor}). 
For multi-horizon architectures, \cite{Lambert_2021} suggested a model that takes the prediction horizon and the current policy’s parameters as input, instead of the full action sequence. Meanwhile, \cite{Whitney_2019} used a dynamic-horizon architecture by padding the shorter action sequences with zeros to fit the input size constraint.

\paragraph{Compounding errors in MBRL} There are many \Grep{papers that study}{works studying} compounding errors and suggest\Gadd{ing} ways to mitigate them. 
\cite{Lambert_2022} showed that the physical system’s stability affects the error profile of a model. 
\cite{Talvitie_2014} proposed \textit{hallucinated replay}, which trains the model with its own generated transitions. 
This technique teaches the model to recover from its own errors, and produces models that have lower 1-step accuracy but higher returns in some scenarios. 
A similar idea (multi-step error) is used by \cite{Byravan_2021} to train models in the context of \Grep{Model-Predictive Control (MPC)}{MPC} \Gadd{MPC was already mentioned before :)}, and \cite{Venkatraman_2015} by casting the error-recovery task as imitation learning. 
In the same \Mrep{optic}{vein},  \cite{Xiao_2023} learned a criterion based on the model’s h-step error, and adjusted the planning horizon accordingly.

% Nevertheless, few papers addressed multi-horizon architectures. \cite{Lambert_2021} suggested a model that takes the prediction horizon and the current policy’s parameters as input, instead of the full action sequence. This method is restricted to simple controllers whose parameters can be fed to a neural network. \cite{Whitney_2019} used a dynamic-horizon architecture by padding the shorter action sequences with zeros to fit the input size constraint. However, this was not studied extensively as it was a practical relaxation used for experiments.
